Machine Learning for the Geosciences: Challenges and Opportunities

Geosciences is a field of great societal relevance that requires solutions to several urgent problems facing our humanity and the planet. As geosciences enters the era of big data, machine learning (ML) -- that has been widely successful in commercial domains -- offers immense potential to contribute to problems in geosciences. However, problems in geosciences have several unique challenges that are seldom found in traditional applications, requiring novel problem formulations and methodologies in machine learning. This article introduces researchers in the machine learning (ML) community to these challenges offered by geoscience problems and the opportunities that exist for advancing both machine learning and geosciences. We first highlight typical sources of geoscience data and describe their properties that make it challenging to use traditional machine learning techniques. We then describe some of the common categories of geoscience problems where machine learning can play a role, and discuss some of the existing efforts and promising directions for methodological development in machine learning. We conclude by discussing some of the emerging research themes in machine learning that are applicable across all problems in the geosciences, and the importance of a deep collaboration between machine learning and geosciences for synergistic advancements in both disciplines.

==> GEO_problems_in_ML.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Geoscience Tasks for Machine Learning}
\label{GEO_problems_in_ML_sec}

 In geoscience problems, the bidirectional coupling of scientific knowledge and observational data has been recognized as being dynamic and data driven \cite{S1,S18}. Many dynamic data driven Earth system applications are emerging from using data to constrain numerical models \cite{S14,S2,S5,S7,S8,S12}, targeting observations with models \cite{S15}, learning from model-data and observations \cite{S10}, and fusing data-driven and numerical models \cite{S5,S6,S7}. Machine learning can play a key role in this transformation by producing symbiotic physics-data systems that use scientific knowledge and the information contained in data respecting their uncertainties. Physically-based machine learning approaches have already advanced numerical models \cite{S4,S7} and machine intelligence \cite{S9} simultaneously.  However, key issues remain.

Geoscience tasks can be categorized as estimation (of the current state of the Earth System) \cite{S2,S4,S5,S7,S8,S10}, parameterization (of fine scale details and “missing knowledge”), prediction (future, short and long term evolution with quantified uncertainty) \cite{S1},  observation (intelligently observing the Earth)\cite{S1,S6}, characterization (of the features that Earth system processes can produce) and discovery (of new dynamical features and modes of behavior), and decision making (making policy choices under change and uncertainty) \cite{S3}. In this section, we discuss these broad categories of problems in geoscience applications highlighting potential for using machine learning methodologies.
\\[0.3cm]
%
{\bf Estimation:}
%
A number of estimation tasks emerge in geoscience for the states and parameters of a physical or empirical model. These applications include numerical weather prediction, paleoclimate, hydrology, solid Earth, and climate modeling, among many others. In many cases, the problems are time dependent, modeled as a dynamical system with imperfect states and parameters, and observed non-uniformly with noise and great sparsity. Modern probabilistic approaches include ensemble methods, with advances towards non-parametric sequential Bayesian inference, e.g. Particle Filters \cite{S1}. There is a great need for developing methodologies that can represent the nonlinear inference problems without sampling in high dimensions and in dealing with model imperfections and sparse data.  Machine learning can play a role in developing tractable Information Theoretic Learning \cite{S5} to reduce sampling burdens in inference, ensemble learning to deal with model error \cite{S2}, scale-recursive graphical models to capture multi-scale multi-rate spatio-temporal mutual information \cite{S17}, use of semi-Markov models for capturing multiple orders of dependencies in time  \cite{levinson1986continuously, heiga2007hidden}, and deep learning methodologies such as long-short term memory (LSTM) models to incorporate the effects of memory at different scales \cite{sak2014long} and the use of statistical-physical models~\cite{S12}.
\\[0.3cm]
%
{\bf Parameterization:}
%
The parameterization problem (e.g., in convection or turbulence)  refers to the fact that the physical processes have infinite scales, but numerical realizations must truncate them at finite scales to be computable. This leaves open the question of what to do about the unrepresented scales, typically finer scales smaller than the grid resolution used for modeling. Parameterizations can be knowledge-based or empirical, which respectively remain expensive and unsatisfactory. Machine learning can play a key role in efficacious parameterization. 
\\[0.3cm]
%
{\bf Prediction:}
%
The long-term predictions of the the Earth system is one of predicting a non-stationary process. A key challenge is to develop approaches that can represent and propagate prediction uncertainties, particularly difficult due to high-dimensionality and nonlinearity~\cite{S1,S11}. In the climate scenario, there is limited long-term predictability at fine scales; increasing resolution does not necessarily improve it, but predictability at the coarse level may also be adversely affected. Approaches to detect key dynamical features and scales are needed together with simplified stochastic model synthesis techniques. Some advances have been made in dynamical downscaling by abstracting dynamics, for example, by using physically-based Markov Chain and Random Field models \cite{S12}, but much remains to be done.  Machine learning models tuned to predictability time-scales of dynamical features remains a key area of impact.
\\[0.3cm]
%
{\bf Observation:}
%
Geoscience processes remain poorly observed, and there is a great opportunity for machine learning methods to infer geoscience variables for cross modal inference \cite{S13}, inferring variables that are difficult to observe directly (e.g., methane concentrations in air or groundwater seepage in soil) using other physical variables (e.g., those observed directly using Earth observing satellites). Machine learning algorithms can be used to analyze remote sensing data and produce estimates of ecosystem variables such as forest cover, health of vegetation, water quality, and surface water availability. There is also a great opportunity for intelligent sensing to adaptively gather data \cite{S6} and control the instrumentation of in-situ sensors to match the evolving dynamical regime of geoscience processes.
\\[0.3cm]
%
{\bf Characterization:}
%
Machine learning algorithms can also help in characterizing objects, events, and processes in geoscience that are critical for understanding the Earth system. For example, we can analyze patterns in geoscience data sets to detect climate events such as tsunamis, cyclogenesis, and tornadogenesis, characterize their features and statistics (e.g., coherent structures \cite{S4,S7,S11}), and discover precursors to such events that can help in predicting them with long leads in time. Mining geoscience data for interesting relationships between features or explanations for current modes (e.g. ENSO) and their impacts is a key challenge. Machine learning can play a key role in the discovery of geoscience features, e.g. the discovery of simplified models, climate teleconnections using network-based algorithms on sea level pressure data \cite{kawale2013graph}.  Causal discovery has recently been applied in the geosciences to identify potential cause-effect relationships from observed data \cite{ED:2012,ED:2017}.

Remote sensing variables can also be used to detect ecosystem changes, which can help in monitoring the Earth's system and contrain physics-based models. In many characterization applications, it is not possible to obtain gold-standard labels that cover the entire range of processes at a global scale. Hence, there is a potential for semi-supervised and unsupervised machine learning methods that can automatically identify patterns, relationships, and anomalies from the data. For example, unsupervised techniques for finding patterns in sea surface height data \cite{faghmous2013parameter,faghmous2014spatio} have resulted in a global mesoscale ocean eddy data set \cite{faghmous2015daily}.
\\[0.3cm]
%
{\bf Decision Making:}
%
Many of the Earth systems in geoscience applications are affected by human actions, thus introducing the need for integrating policy actions in the modeling approaches. The outputs produced by geoscience models can help inform policy  and decision making. 
The science of causal attribution is an essential tool for decision making that helps scientists determine the causes of events \cite{causal_attribution,ED:2012}.
Of great interest is the development of decision methodology with uncertain prediction probabilities, producing ambiguous risk with poorly resolved tails representing the most interesting extreme, rare, and transient events produced by models. The application of reinforcement learning and other stochastic dynamic programming approaches that can solve decision problems with ambiguous risk \cite{S3} is a needed advance that machine learning can pursue.





==> ML_section.tex <==

\section*{Acknowledgements}

The 2015 NSF-funded workshop on {\it Intelligent and Information  Systems for Geosciences} (IS-GEO) was the brain child of the two workshop chairs,
Yolanda Gil and Suzanne A Pierce. 
The participants of the workshops were 
Hassan Babaie, %Georgia State University
Arindam Banerjee, %University of Minnesota
Kirk Borne, %George Mason University
Gary Bust, %Johns Hopkins
Michelle Cheatham, %Wright State University
Imme Ebert-Uphoff, %Colorado State University
Carla Gomes, %Cornell University
Mary Hill, %The University of Kansas
John Horel, %University of Utah
Leslie Hsu, %Columbia University
Jim Kinter, %George Mason University
Craig Knoblock, %University of Southern California
David Krum, %University of Southern California
Vipin Kumar, %University of Minnesota
Pierre Lermusiaux, %Massachusetts Institute of Technology
Yan Liu, %University of Southern California
Deborah McGuinness, %Rensselaer Polytechnic Institute
Chris North, %Virginia Tech
Victor Pankratius, %Massachusetts Institute of Technology
Shanan Peters, %University of Wisconsin-Madison
Beth Plale, %Indiana University Bloomington
Allen Pope, %University of Colorado Boulder
Sai Ravela, %Massachusetts Institute of Technology
Juan Restrepo, %Oregon State University
Aaron Ridley, %University of Michigan
Hanan Samet, %University of Maryland
Shashi Shekhar, %University of Minnesota
Katie Skinner, %University of Michigan
Padhraic Smyth, %University of California, Irvine
Basil Tikoff, %University of Wisconsin-Madison
Lynn Yarmey, %National Snow and Ice Data Center
and Jia Zhang. %Carnegie Mellon University – Silicon Valley
We thank the NSF for funding this workshop under grant {\color{red} NSF-XXX}.


==> Opportunities_for_ML.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Promising Recent Machine Learning Advances}
\label{Opportunities_for_ML_sec}

In this section, we focus on some of the recent advances in machine learning research that have received considerable attention in several real-world applications and are directly pertinent for addressing some of the pressing challenges in analyzing geoscience data. This includes: (i) Learning in nonlinear high-dimensional inference~\cite{S1}, (ii) multi-task learning for addressing heterogeneity in geoscience data across space and time, (iii) multi-instance and multi-view learning for handling data from different sources at multiple spatial and temporal resolutions, and (iv) active learning and semi-supervised learning methods for handling the paucity of labeled data. 
Some of these machine learning advances have been discussed in the context of monitoring land cover changes using remote sensing data in \cite{Karpatne:2016}.
We provide a brief overview of each of these machine learning advances in the following.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Learning Nonlinear High-Dimensional Inference Under Uncertainty}

Some fundamental challenges underpin Geoscience problems including nonlinearity of the  processes, high-dimensionality of  models, and complex non-Gaussian error uncertainties in data, initial conditions, parameters and parameterization. Further, the data is sparse, and the uncertainty distributions remain poorly sampled~\cite{S11,S1}. Effective inference for these variables benefit from recent advances in machine learning, such as using tractable information theoretic learning~\cite{S5}, manifold learning, ensemble learning~\cite{S2} and transfer learning. The success of these methods emerges by embedding them in two-way interactions between models and data; using data to constrain numerical or empirical models and in reverse using the models to target data~\cite{S1,S18}. This paradigm provides novel framework for ML-Geo symbiosis bu facilitating feedback between data-driven and theory-driven models.

\subsection{Multi-task Learning for Addressing Heterogeneity in Data}

The goal of multi-task learning is to improve the predictive performance over several tasks by exploiting the commonalities among related tasks \cite{baxter2000model,caruanamultitask,pan2010survey}, especially when some tasks suffer from paucity of training samples. As an example, consider the problem of detecting ecosystem changes such as forest fires using geoscience observations such as multi-spectral reflectance data from Earth observing satellites. As discussed in Section 3, the presence of varying geographies, topographies, and land cover types directs the need for learning a different model for every homogeneous region in the world, which can be considered as a separate learning task. If we had sufficient number of training samples at every task (every homogeneous partition in geoscience data), we could have independently learned a separate model for every learning task. However, as described in Section 3, this is not the case in a number of real-world geoscience applications suffering from paucity of training data, which can result in overfitting at the individual tasks when considered individually. To account for the heterogeneity in geoscience processes without getting affected by the paucity of training data, multi-task learning provides a solution for sharing the models across tasks that are similar to each other, thus increasing robustness and avoiding overfitting across such tasks.  An example of a multi-task learning based approach for handling heterogeneity can be found in a recent work in \cite{karpatnepredictive2014}, where the learning of a forest cover model at every vegetation type (discovered by clustering vegetation time-series at locations) was treated as a separate task, and the similarity among vegetation types (extracted using hierarchical clustering techniques) was used to share the learning at related tasks.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Multi-instance and Multi-view Learning for Analyzing Multi-resolution Data}

In multi-instance learning, the basic unit of classification is not an individual instance but a bag of multiple instances, where every bag has an associated class label \cite{dietterich1997solving}. Multi-instance learning is a natural paradigm for handling scenarios in geoscience where the training labels are available at coarser resolutions in space and time than the actual observations, e.g., due to the high costs in obtaining high resolution ground-truth labels. For example, ground-truth information of forest fire events are generally available as spatially detailed polygons but only at annual scales, without any information about the exact time of occurrence of the fire. In such a setting, the sequence of observations at a pixel within a year can be considered as a bag of instances, where every bag (year) has an associated binary label (burned or unburned), motivating the use of a multi-instance learning framework. Another scenario where we can use multi-instance learning to handle differences in resolution between observations and ground-truth labels is when the observations are available at fine spatial resolutions, but ground-truth information is available at spatially coarse resolutions, e.g., at spatially coarse grids superimposed on the high-resolution observations. This line of work was explored by Vatsavai et al.\ \cite{vatsavai2013gaussian,vatsavai2013object} for distinguishing informal settlements (slums) from formal urban settlements using very high resolution (VHR) remote sensing datasets, where the ground-truth labels were annotated by human experts at coarse spatial resolutions. 

Another machine learning paradigm that can possibly help in handling the challenges in integrating information from data collected via multiple sources (e.g., satellite sensors) is multi-view learning. The multi-view learning paradigm is useful when there are multiple diverse views of the same object (e.g., from different sources), and there is a limited supply of training instances but there is an ample supply of unlabeled instances. In such a case, the multi-view learning paradigm provides a unique way of leveraging information from various views of the data while ensuring that the predictions on the unlabeled data obtained from the different views are consistent with each other. Multi-view learning can be applied in many geoscience applications where there is sufficient supply of unlabeled instances, e.g. those obtained from high-resolution remote sensing products that are used for monitoring ecosystem changes such as deforestation, forest fires, and changes in surface water bodies.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Active Learning and Semi-supervised Learning for Handling Paucity of Labels}

Semi-supervised learning, also known as classification with labeled and unlabeled data, is a popular machine learning technique designed to deal with small training sample problems in supervised learning. The popularity of semi-supervised approaches \cite{ssl-survey} can be attributed to the fact that several studies have reported improved classification accuracies and that unlabeled training samples are often readily available. Semi-supervised is suitable in geoscience applications where we can leverage the structure in unlabeled observations for improving the learning of machine learning models, even when we have limited number of training samples. A related area of research that attempts to address the paucity of training data is active learning \cite{settles2010active}, where the idea is to actively involve a human annotator in the process of training an effective machine learning model. The goal of active learning is to request the smallest number of annotations from the expert, e.g., sampling difficult instances at the boundaries of the classes, in order to learn a model with sufficiently reasonable accuracy.  Both active learning and semi-supervised learning frameworks can be used in conjugation with many machine learning algorithms for handling the paucity of training data in different problem settings.




==> Vision.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Vision for a Deeply Integrated Geoscience-guided Machine Learning Paradigm}
\label{Vision_sec}

The basic goal in most geoscience applications is to represent relationships between variables, e.g., the effect of carbon emission on the global dynamics of climate variables such as temperature. This is achieved with the help of physics-based models that either involve solving closed-form equations or running computational simulations of dynamical systems. Despite the usefulness of physics-based models in explaining several geoscience processes, they suffer from certain knowledge gaps in problems where our current physical understanding is limited mainly because of the inherent complexity of the processes, e.g., the flow and transport of groundwater beneath the Earth's surface or the physics behind the creation and movement of clouds. In such settings, physics-based models are often forced to make many parametric approximations about the physical processes, which not only leads to poor predictive performance but also renders the model difficult to comprehend and analyze.

An alternate possibility is to automatically learn relationships between geoscience variables using data science models, which have found great success in commercial applications and are rapidly transforming the way we extract knowledge from large data sets in vision and speech. However, solely relying on the knowledge contained in the limited number of data samples can lead to physically inconsistent models that are not only uninterpretable but also suffer from poor predictive performance due to the phenomena of overfitting. Hence, neither a data-only nor a physics-only approach can be considered sufficient for knowledge discovery in complex scientific applications such as geoscience. Instead, there is an opportunity in pursuing an alternate paradigm of research that explores the continuum between theory-based and data science models by deeply integrating scientific knowledge with data science methodologies. This is the paradigm of theory-guided data science that is beginning to be pursued in several scientific disciplines ranging from material science to hydrology, turbulence modeling, and biomedicine. A recent paper \cite{tgds} builds the foundation of this paradigm and illustrates several ways of blending scientific knowledge with data science models using emerging applications from diverse domains. There is a great opportunity in exploring similar lines of research in geoscience applications, where machine learning methods can play a major role in accelerating knowledge discovery by automatically learning patterns and models from the data, but without ignoring the wealth of knowledge accumulated in physics-based model representations of geoscience processes.

In geoscience problems, the fully coupled nature of scientific knowledge and observational data is recognized \cite{S1}. Traditionally, observations have seeded theory, but increasingly our inferences rely on their computational models whose effectiveness also depends on being constrained by observations.  We note that in reverse, models offer the prospect of intelligent information gathering so that a bidirectional coupling is central \cite{S18}. Geoscience is indeed evolving from using data to constrain models \cite{S14,S2,S5,S7,S8,S12}, targeting observations with models \cite{S15}, using model-data as observations \cite{S1}, inducing models from observations \cite{S10}, and fusing data-driven and numerical models \cite{S5,S6,S7}, e.g., dynamic data driven Earth system applications \cite{S1}. Machine learning can play a key role in this transformation to result in hybrid-physics-data systems that use scientific knowledge and the knowledge contained in data at an equal footing. Physically-based machine learning approaches have already advanced numerical models \cite{S4,S7} and machine intelligence \cite{S9} simultaneously. Machine learning can also provide an objective data-driven basis for understanding mechanisms of physical processes, that can further our scientific understanding of geoscience phenomena. 

==> references.tex <==
%%%%%%%%%%%%% BIBLIOGRAPHY %%%%%%%%%%%%%%%

\begin{thebibliography}{99}


\bibitem{S10}	
E. Basha, S. Ravela and D. Rus, 
{\em Model-based Monitoring for Early Warning Flood Detection}, 
Proc. 6th  ACM Conf. on Embedded Networked Sensor Systems, pp. 295-308, 2008.

\bibitem{baxter2000model}
  {J.\ Baxter},
  {\em A model of inductive bias learning},
  {J. Artif. Intell. Res.(JAIR)},
  vol.\ {12},
  pp.\ {149--198},
  {2000}.

\bibitem{caruanamultitask}
  {R.\ Caruana},
  {\em Multitask Learning: A Knowledge-Based Source of Inductive Bias},
  {Proceedings of the Tenth International Conference on Machine Learning},
  pp.\ {41--48},
  1993.
  %organization={Citeseer}

\bibitem{Carbone:2016}A.\ Carbone, M.\ Jensen, and A.-H.\ Sato,
{\em Challenges in data science: a complex systems perspective},
2016.


\bibitem{S18}	
F. Darema, 
{\em Dynamic Data Driven Applications Systems: A New Paradigm for Application Simulations and Measurements}, LNCS 3038:662-669, 2004.

\bibitem{dietterich1997solving}
  {T.G.\ Dietterich, and R.H.\ Lathrop, and T.\ Lozano-P{\'e}rez},
  {\em Solving the multiple instance problem with axis-parallel rectangles},
  {Artificial intelligence},
  vol.\ {89},
  no.\ {1},
  pp.\ {31--71},
  {1997}.
  %publisher={Elsevier}


\bibitem{ED:2012}
I. Ebert-Uphoff, Y. Deng,
{\em Causal Discovery for Climate Research Using Graphical Models},
Geophysical Research Letters, vol. 39, L19701, 7 page, 2012.  
  
\bibitem{ED:2017}	
I. Ebert-Uphoff and Y. Deng,
{\em Causal Discovery in the geosciences - Using synthetic data to learn how to interpret results}, 
Computer \& Geosciences, Vol.\ 99, Feb.\ 2017, pp.\ 50-60.


\bibitem{S12}	
K. Emanuel, S. Ravela, C. Risi, and E. Vivant, 
{\em A Statistical Deterministic Approach to Hurricane Risk Assessment}, 
Bulletin of American Meteorological Society, 87(3): 299-314, 2006



\bibitem{faghmous2015computing}
J.~H. Faghmous, V.~Kumar, and S.~Shekhar, ``Computing and climate,''
  \emph{Computing in Science \& Engineering}, vol.~17, no.~6, pp. 6--8, 2015.

\bibitem{faghmous2014big}
J.~H. Faghmous and V.~Kumar, ``A big data guide to understanding climate
  change: The case for theory-guided data science,'' \emph{Big data}, vol.~2,
  no.~3, pp. 155--163, 2014.

\bibitem{faghmous2013parameter}
J.~H. Faghmous, M.~Le, M.~Uluyol, V.~Kumar, and S.~Chatterjee, ``A
  parameter-free spatio-temporal pattern mining model to catalog global ocean
  dynamics,'' in \emph{Data Mining (ICDM), 2013 IEEE 13th International
  Conference on}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2013, pp.
  151--160.

\bibitem{faghmous2014spatio}
J.~H. Faghmous, H.~Nguyen, M.~Le, and V.~Kumar, ``Spatio-temporal consistency
  as a means to identify unlabeled objects in a continuous data field.'' in
  \emph{AAAI}, 2014, pp. 410--416.

\bibitem{faghmous2015daily}
J.~H. Faghmous, I.~Frenger, Y.~Yao, R.~Warmka, A.~Lindell, and V.~Kumar, ``A
  daily global mesoscale ocean eddy dataset from satellite altimetry,''
  \emph{Scientific data}, vol.~2, 2015.
  
  
\bibitem{causal_attribution}
A.\ Hannart, J.\ Pearl, F.E.L.\ Otto, P.\ Naveau, and M.\ Ghil,
{\em Causal Counterfactual Theory for the Attribution of Weather and Climate-Related Events},
Bulletin of the American Meteorological Society, Jan 2016.


\bibitem{IS-GEO:1995}  Y. Gil et al., {\it Final workshop report}, 2015 Workshop on Intelligent and Information Systems for Geosciences, Nov 2015, available at 
\url{https://isgeodotorg.files.wordpress.com/2015/12/} 
\url{is-geo-report_30november2015-final.pdf}.

\bibitem{heiga2007hidden}
  {Z.\ Heiga, K.\ Tokuda, T.\ Masuko, T.\ Kobayasih, and T.\ Kitamura},
  {\em A hidden semi-Markov model-based speech synthesis system},
  {IEICE Transactions on Information and Systems},
  vol.\ 90,
  no.\ 5,
  pp.\ 825--834,
  2007.
  %publisher={The Institute of Electronics, Information and Communication Engineers}


\bibitem{Karpatne:2016}
A. Karpatne, Z. Jiang, R.R. Vatsavai, S. Shekhar, and V. Kumar, 
{\em Monitoring Land-Cover Changes}, 
IEEE Geoscience and Remote Sensing Magazine, June 2016.


\bibitem{karpatne2013earth}
A.~Karpatne, J.~Faghmous, J.~Kawale, L.~Styles, M.~Blank, V.~Mithal, X.~Chen,
  A.~Khandelwal, S.~Boriah, K.~Steinhaeuser \emph{et~al.}, ``Earth science
  applications of sensor data,'' in \emph{Managing and Mining Sensor
  Data}.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 2013, pp. 505--530.

\bibitem{karpatne2015guide}
A.~Karpatne and S.~Liess, ``A guide to earth science data: Summary and research
  challenges,'' \emph{Computing in Science \& Engineering}, vol.~17, no.~6, pp.
  14--18, 2015.
  
\bibitem{tgds}
  {A.\ Karpatne, G.\ Atluri, J.\ Faghmous, M.\ Steinbach, A.\ Banerjee, A.\ Ganguly, S.\ Shekhar, N.\ Samatova, and V.\ Kumar},
  {\em Theory-guided data science: A new paradigm for scientific discovery},
  %{IEEE Transactions on Knowledge and Data Engineering (in review)}, 
  arXiv: 1612.08544,
  2017.
  
\bibitem{karpatnepredictive2014}
  {A.\ Karpatne, A.\ Khandelwal, S.\ Boriah, S.\ Chatterjee and V.\ Kumar},
  {\em Predictive learning in the presence of heterogeneity and limited training data},
  {Proceedings of the 2014 SIAM International Conference on Data Mining},
  pp.\ {253--261},
  {2014}.
  
  
\bibitem{kawale2013graph}
  J.\ Kawale, S.\ Liess, A.\ Kumar, M.\ Steinbach, P.\ Snyder, V.\ Kumar, A.R.\ Ganguly, N.F.\ Samatova, and F.\ Semazzi,
  {\em A graph-based approach to find teleconnections in climate data},
  {Statistical Analysis and Data Mining: The ASA Data Science Journal},
  Wiley Online Library,
  vol.\ 6,
  no.\ 3,
  pp.\ 158--179,
  2013.
  

\bibitem{Lary:2016}D.J.\ Lary, A.H.\ Alavi, A.H.\ Gandomi, and A.L.\ Walker, {\it Machine Learning in geosciences and remote sensing}, Geoscience Frontiers 7, 3-10, 2016.

\bibitem{levinson1986continuously}
  S.E.\ Levinson,
  {\em Continuously variable duration hidden Markov models for automatic speech recognition},
  {Computer Speech \& Language},
  vol.\ 1,
  no.\ 1,
  pp.\ 29--45,
  1986.
  %publisher={Elsevier}

\bibitem{S16}	
E. N. Lorenz, 
{\em Deterministic Nonperiodic Flow}, 
Journal of the Atmospheric Sciences. 20 (2): 130–141, 1963.

\bibitem{S15}	
E. N. Lorenz, and K.A. Emanuel, 
{\em Optimal sites for supplementary weather observations: Simulations with a small model}, 
J. Atmos. Sci., 55, 399-414, 1998.



\bibitem{CI:2013}C.\ Monteleoni, G.A.\ Schmidt, F.\ Alexander, A.\ Niculescu-Mizil, K.\ Steinhaeuser, M.\ Tippett, A.\ Banerjee, M.B.\ Blumenthal, A.R.\ Ganguly, J.E\. Smerdon, and M.\ Tedesco, 
{\em Climate informatics}, In Computational Intelligent Data Analysis for Sustainable Development; Data Mining and Knowledge Discovery Series, Chapman and Hall/CRC, 81-126, 2013.
%http://faculty.cs.gwu.edu/~cmontel/ciBookChapter.pdf

\bibitem{CI:2016}C.\ Monteleoni, G.A.\ Schmidt, S.\ McQuade, 
{\em Climate Informatics: Accelerating Discovering in Climate Science with Machine Learning}, Computing in Science \& Engineering 15, 32 (2016); 
\url{doi: http://dx.doi.org/10.1109/MCSE.2013.50}.

\bibitem{pan2010survey}
  {S.J.\ Pan and Q.\ Yang},
  {\em A survey on transfer learning},
  {Knowledge and Data Engineering, IEEE Transactions on},
  vol.\ {22},
  no.\ {10},
  pp.\ {1345--1359},
  {2010}.
  %publisher={IEEE}


\bibitem{S11}	
S. Ravela, 
{\em Amplitude-Position Formulation of Data Assimilation}, 
LNCS 3993:497-505, 2006.

\bibitem{S4}	
S. Ravela, 
{\em A Statistical Theory of Inference for Coherent Structures}, 
LNCS 8964: 121–133, 2015

\bibitem{S7}	
S.\ Ravela, 
{\em Quantifying Uncertainty for Coherent Structures}, 
Procedia Computer Science, vol. 9, pp. 1187–1196, 2012.

\bibitem{S1}	
S.\ Ravela and A.\ Sandu (Eds.), {\em Dynamic Data-driven Environmental Systems Science (DyDESS)}, vol. 8964: Springer, 2015.

\bibitem{S8}	
S. Ravela, J. Marshall, C. Hill, A. Wong and S. Stransky, 
{\em A Realtime Observatory for Laboratory Simulation of Planetary Flows, Experiments in Fluids}, 
48(5):915-925, 2010.

\bibitem{S6}	
S. Ravela, I. Sleder and J. Salas, 
{\em Mapping Coherent Atmospheric Structures with Small Unmanned Aircraft Systems}, Infotech@Aerospace, AIAA, 2013

\bibitem{S3}	
S.\ Ravela, C.\ Denamiel, H.\ Jacoby and J.\ Holak, 
{\em Quantifying Uncertainty and Uncertain Probabilities in Hurricane Induced Risk Assessment and Mitigation Planning Under a Changing Climate}, 
5th International Conference on Hurricanes and Climate, Chania, Greece, 2015

\bibitem{S13}	
S. Ravela, A. Torralba and W. T. Freeman, 
{\em An Ensemble Prior of Image Structure for Cross-modal Inference}, 
ICCV 1:871-876, 2005.

\bibitem{sak2014long}
  {H.\ Sak, A.W.\ Senior, and F.\ Beaufays},
  {\em Long short-term memory recurrent neural network architectures for large scale acoustic modeling.},
  {INTERSPEECH},
  pp.\ 338--342,
  2014.

\bibitem{settles2010active}
  {B.\ Settles},
  {\em Active learning literature survey},
  {Comp.\ Science Tech.\ Rep.\ 1648},
  {University of Wisconsin, Madison},
  {2010}

\bibitem{S2}	
H.\ Seybold, S.\ Ravela and P.\ Tagade, 
{\em Ensemble Learning in Non-Gaussian Data Assimilation}, 
LNCS 8964: 227-238, 2015.

\bibitem{siegert2001increased}
  F.\ Siegert, G.\ Ruecker, A.\ Hinrichs, and A.A.\ Hoffmann,
  {\em Increased damage from fires in logged forests during droughts caused by El Ni\~{n}o},
  {Nature}, 
  vol.\ 414,
  no.\ 6862,
  pp.\ 437--440,
  year={2001}.


\bibitem{Stillings:2012}N.\ Stillings, N., {\it Complex systems in the geosciences and in geoscience learning}, Geological Society of America Special Papers, 486, 97-111, 2012.

\bibitem{S17}	
E.B.\  Sudderth,  M.J.\  Wainwright,  and  A.S.\  Willsky,  
{\em Embedded Trees: Estimation of Gaussian processes on graphs with cycles}, 
IEEE Transactions  on  Signal  Processing,  vol.  52,  no.  11,  pp.  3136–3150, November 2004.


\bibitem{S5}	
P. Tagade and S. Ravela, 
{\em On a Quadratic Measure of Mutual Information for Data Assimilation}, 
IEEE ACC, pp. 598 – 603, DOI: 10.1109/ACC.2014.6859127, 2014

\bibitem{Thompson1}
D.\ R.\ Thompson, I.\ Leifer, H.\ Bovensmann, M.\ Eastwood, M.\ Fladeland, C.\ Frankenberg, K.\ Gerilowski et al.,
{\em Real-time remote detection and measurement for airborne imaging spectroscopy: a case study with methane}, 
Atmospheric Measurement Techniques 8, no. 10 (2015): 4383-4397.


\bibitem{vatsavai2013gaussian}
  {R.R.\ Vatsavai},
  {\em Gaussian multiple instance learning approach for mapping the slums of the world using very high resolution imagery},
  {Proceedings of the 19th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pp.\ ={1419--1426},
  {2013}.
  %organization={ACM}

\bibitem{vatsavai2013object}
  {R.R.\ Vatsavai},
  {\em Object based image classification: state of the art and computational challenges},
  {Proceedings of the 2nd ACM SIGSPATIAL International Workshop on Analytics for Big Geospatial Data},
  pp.\ {73--80},
  {2013}.
  %organization={ACM}

\bibitem{wallace1981teleconnections}
   J.M.\ Wallace, J.M.\ Gutzler, S.\ David,
  {\em Teleconnections in the geopotential height field during the Northern Hemisphere winter},
  Monthly Weather Review,
  vol.\ 109,
  no.\ 4,
  pp.\ 784--812,
  1981.
  
\bibitem{ward2014strong}
  P.J.\ Ward, B.\ Jongman, M.\ Kummu, M.D.\ Dettinger, and F.C.\ Sperna Weiland and H.C.\ Winsemius,
  {\em Strong influence of El Ni\~{n}o Southern Oscillation on flood risk around the world},
  {Proceedings of the National Academy of Sciences},
  vol.\ 111,
  no.\ 44,
  pp.\ 15659--15664,
  2014.
  %publisher={National Acad Sciences}
  
  

\bibitem{S14}	
C. Wunsch, 
{\em Discrete Inverse and State Estimation Problems With Geophysical Fluid Applications}, 
Cambridge University Press, 371 pp., 2006.

\bibitem{S9}	
C.\ Yang, and S. Ravela, 
{\em Deformation Invariant Image Matching by Spectrally Controlled Diffeomorphic Alignment}, 
IEEE ICCV, pp. 1303-1310, 2009.

\bibitem{Yeh:2015}  T-C.\ Yeh, R.\ Khaleel, R., and K.C.\ Carroll, K. C., 
{\em Flow Through Heterogeneous Geologic Media}, 
Cambridge University Press, 2015.  


\bibitem{ssl-survey}
            {X.\ Zhu},
            {\em Semi-Supervised Learning Literature Survey},
            {Tech.\ Rep.\ No.\ 1530},
            {University of Wisconsin},
            {December, 2007},
            \url{http://pages.cs.wisc.edu/~jerryzhu/pub/}
		\url{ssl_survey.pdf}.






%\bibitem{Thompson2}
%C.\ Frankenberg, A.K.\ Thorpe, D.R.\ Thompson, G.\ Hulley, E.A.\ Kort, N.\ Vance, J.\ Borchardt et al., 
%{\em Airborne methane remote measurements reveal heavy-tail flux distribution in Four Corners region}, 
%Proceedings of the National Academy of Sciences (2016): 201605617.


%\bibitem{NCEP-NCAR:1996}E.\ Kalnay, M. Kanamitsu, R. Kistler, W. Collins, D. Deaven, L. Gandin, M. Iredell, S. Saha, G. White, J. Woollen, Y. Zhu, M. Chelliah, W. Ebisuzaki, W. Higgins, J. Janowiak, K. C. Mo, C. Ropelewski, J. Wang, A. Leetmaa, R. Reynolds, R. Jenne, and D. Joseph, {\em The NCEP/NCAR 40-Year Reanalysis Project}, Bull. Amer. Meteor. Soc., 77, 437–471, 1996.

%\bibitem{NCEP-NCAR:2001}R.\ Kistler, E. Kalnay, W. Collins, S. Saha, G. White, J. Woollen, M. Chelliah, W. Ebisuzaki, M. Kanamitsu, V. Kousky, H. van den Dool, R. Jenne, and M. Fiorino, {\em The NCEP-NCAR 50-Year Reanalysis: Monthly Means CD-ROM and Documentation}, Bull. Amer. Meteor. Soc., 82, 247–268, 2001.


%\bibitem{DE:2014}
%Y.\ Deng, I.\ Ebert‐Uphoff, 
%{\em Weakening of Atmospheric Information Flow in a Warming Climate in the Community Climate System %Model}, 
%Geophysical Research Letters, 7 pages, Jan 2014.




%%%%%%% SORTED UP TO HERE %%%%%%%%%



\end{thebibliography}











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\remove{

% References from Anuj in bibtex format:

%--------------------------
@article{wallace1981teleconnections,
  title={Teleconnections in the geopotential height field during the Northern Hemisphere winter},
  author={Wallace, John M and Gutzler, David S},
  journal={Monthly Weather Review},
  volume={109},
  number={4},
  pages={784--812},
  year={1981}
}
%--------------------------
@article{kawale2013graph,
  title={A graph-based approach to find teleconnections in climate data},
  author={Kawale, Jaya and Liess, Stefan and Kumar, Arjun and Steinbach, Michael and Snyder, Peter and Kumar, Vipin and Ganguly, Auroop R and Samatova, Nagiza F and Semazzi, Fredrick},
  journal={Statistical Analysis and Data Mining: The ASA Data Science Journal},
  volume={6},
  number={3},
  pages={158--179},
  year={2013},
  publisher={Wiley Online Library}
}
%--------------------------
@article{siegert2001increased,
  title={Increased damage from fires in logged forests during droughts caused by El Nino},
  author={Siegert, F and Ruecker, G and Hinrichs, A and Hoffmann, AA},
  journal={Nature},
  volume={414},
  number={6862},
  pages={437--440},
  year={2001},
  publisher={Nature Publishing Group}
}
%--------------------------
@article{ward2014strong,
  title={Strong influence of El Nino Southern Oscillation on flood risk around the world},
  author={Ward, Philip J and Jongman, Brenden and Kummu, Matti and Dettinger, Michael D and Weiland, Frederiek C Sperna and Winsemius, Hessel C},
  journal={Proceedings of the National Academy of Sciences},
  volume={111},
  number={44},
  pages={15659--15664},
  year={2014},
  publisher={National Acad Sciences}
}
%--------------------------
@article{levinson1986continuously,
  title={Continuously variable duration hidden Markov models for automatic speech recognition},
  author={Levinson, Stephen E},
  journal={Computer Speech \& Language},
  volume={1},
  number={1},
  pages={29--45},
  year={1986},
  publisher={Elsevier}
}
%--------------------------
@article{heiga2007hidden,
  title={A hidden semi-Markov model-based speech synthesis system},
  author={Heiga, ZEN and Tokuda, Keiichi and Masuko, Takashi and Kobayasih, Takao and Kitamura, Tadashi},
  journal={IEICE Transactions on Information and Systems},
  volume={90},
  number={5},
  pages={825--834},
  year={2007},
  publisher={The Institute of Electronics, Information and Communication Engineers}
}
%--------------------------
@inproceedings{sak2014long,
  title={Long short-term memory recurrent neural network architectures for large scale acoustic modeling.},
  author={Sak, Hasim and Senior, Andrew W and Beaufays, Fran{\c{c}}oise},
  booktitle={INTERSPEECH},
  pages={338--342},
  year={2014}
}
%--------------------------
@article{pan2010survey,
  title={A survey on transfer learning},
  author={Pan, Sinno Jialin and Yang, Qiang},
  journal={Knowledge and Data Engineering, IEEE Transactions on},
  volume={22},
  number={10},
  pages={1345--1359},
  year={2010},
  publisher={IEEE}
}
%--------------------------
@inproceedings{caruanamultitask,
  title={Multitask Learning: A Knowledge-Based Source of Inductive Bias1},
  author={Caruana, R},
  booktitle={Proceedings of the Tenth International Conference on Machine Learning},
  pages={41--48},
  organization={Citeseer}
}
%--------------------------
@article{baxter2000model,
  title={A model of inductive bias learning},
  author={Baxter, Jonathan},
  journal={J. Artif. Intell. Res.(JAIR)},
  volume={12},
  pages={149--198},
  year={2000}
}
%--------------------------
@inproceedings{karpatnepredictive2014,
  title={Predictive learning in the presence of heterogeneity and limited training data},
  author={Karpatne, Anuj and Khandelwal, Ankush and Boriah, Shyam and Chatterjee, Snigdhansu and Kumar, Vipin},
  booktitle={Proceedings of the 2014 SIAM International Conference on Data Mining},
  pages={253--261},
  year={2014}
}
%--------------------------
@article{dietterich1997solving,
  title={Solving the multiple instance problem with axis-parallel rectangles},
  author={Dietterich, Thomas G and Lathrop, Richard H and Lozano-P{\'e}rez, Tom{\'a}s},
  journal={Artificial intelligence},
  volume={89},
  number={1},
  pages={31--71},
  year={1997},
  publisher={Elsevier}
}
%--------------------------
@inproceedings{vatsavai2013gaussian,
  title={Gaussian multiple instance learning approach for mapping the slums of the world using very high resolution imagery},
  author={Vatsavai, Ranga Raju},
  booktitle={Proceedings of the 19th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={1419--1426},
  year={2013},
  organization={ACM}
}
%--------------------------
@inproceedings{vatsavai2013object,
  title={Object based image classification: state of the art and computational challenges},
  author={R. Vatsavai, R.},
  booktitle={Proceedings of the 2nd ACM SIGSPATIAL International Workshop on Analytics for Big Geospatial Data},
  pages={73--80},
  year={2013},
  organization={ACM}
}
%--------------------------
@techreport{ssl-survey,
            author = {Zhu, Xiaojin},
            month = {December},
            title = {Semi-Supervised Learning Literature Survey},
            url = {http://pages.cs.wisc.edu/~jerryzhu/pub/ssl_survey.pdf},
            institution = {University of Wisconsin},
            volume = {Tech. Rep. No. 1530},
            year = {2007}
}
%--------------------------
@article{settles2010active,
  title={Active learning literature survey},
  author={Settles, Burr},
  journal={University of Wisconsin, Madison},
  volume={52},
  number={55-66},
  pages={11},
  year={2010}
}
%--------------------------
@inproceedings{tgds,
  title={Theory-guided data science: A new paradigm for scientific discovery},
  author={Karpatne, Anuj and Atluri, Gowtham and Faghmous, James and Steinbach, Michael and Banerjee, Arindam and Ganguly, Auroop and Shekhar, Shashi and Samatova, Nagiza and Kumar, Vipin},
  booktitle={IEEE Transactions on Knowledge and Data Engineering (in review), arXiv: 1612.08544},
  year={2017}
}
%--------------------------

}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




